A Simple Construction of Quantum Public-Key Encryption from Quantum-Secure One-Way Functions

Quantum public-key encryption [Gottesman; Kawachi et al., Eurocrypt'05] generalizes public-key encryption (PKE) by allowing the public keys to be quantum states. Prior work indicated that quantum PKE can be constructed from assumptions that are potentially weaker than those needed to realize its classical counterpart. In this work, we show that quantum PKE can be constructed from any quantum-secure one-way function. In contrast, classical PKE is believed to require more structured assumptions. Our construction is simple, uses only classical ciphertexts, and satisfies the strong notion of CCA security.

==> main_proof_backup.tex <==
\begin{proof}[Theorem~\ref{lemma:generic_rewinding_lemma}]
The goal is to define a process which, for any honestly generated public key $pk$, starting with the state $\ket{\psi}\ket{0} = \ket{pk}^{\otimes m}\ket{0}_{aux}$, outputs the state $\Pi_1 U\ket{\psi}\ket{0}$. The idea is to follow a similar approach to the quantum rewinding lemma proof from~\cite{DBLP:journals/siamcomp/Watrous09}. Let $U$, $\Pi$ be defined as before, and define $\Delta = \{\Delta_0 ,\Id - \Delta_0\}$ to be a projective measurement such that $\Delta_0 =\Id \otimes \ket{0}\bra{0}_{aux}$, i.e. a projection unto the space where all auxiliary qubits are set to $0$. Moreover consider the Hilbert space $\mathcal{H}$ to be the Hilbert space spanned by $\{\ket{pk}^{\otimes m}\}$ where $\ket{pk}$'s are honestly generated public keys. Now $U$ can be seen as a unitary on the Hilbert space $\mathcal{H}\otimes (\mathbb{C}^{2})^{\otimes l}$.

Following the notation used in lemma~\ref{lemma:orthonormal_basis}, for all $\ket{\psi}\in \mathcal{H}$ we define, $\phi_0(\psi)$, $\phi_1(\psi)$ and $p(\psi)$ to be the unique vectors and values such that, 
\begin{align*}
    U \ket{\psi}\ket{0} = \sqrt{p(\psi)}\ket{1}_{\text{out}}\ket{\phi_1(\psi)} + \sqrt{1-p(\psi)}\ket{0}_{\text{out}}\ket{\phi_0(\psi)} 
\end{align*}

We further define $\{\psi_i\}_{i \in [1,\dots,k]}$ to be the orthonormal basis of $\mathcal{H}$ induced by the eigenvectors of the operator
$$(\Id \otimes \bra{0})^{\dagger} U^{\dagger} \Pi_1 U (\Id \otimes \ket{0})$$
Now due to lemma~\ref{lemma:orthonormal_basis} we have that $\{\ket{0}\ket{\phi_0(\psi_i)}\}\cup \{\ket{1}\ket{\phi_1 (\psi_i)}\}$ forms an orthonormal basis for the support of $U (\Id\otimes \ket{0})$. This allows us to define a unitary $V$ which acts as follows, 
\begin{align*}
    V(\sqrt{p(\psi_i)} \ket{1}\ket{\phi_1(\psi_i)} + \sqrt{1-p(\psi_i)} \ket{0}\ket{\phi_0(\psi_i)}) = \sqrt{q} \ket{1}\ket{\phi_1(\psi_i)} + \sqrt{1-q} \ket{0}\ket{\phi_0(\psi_i)} \\
    V(\sqrt{1-p(\psi_i)} \ket{1}\ket{\phi_1(\psi_i)} - \sqrt{p(\psi_i)} \ket{0}\ket{\phi_0(\psi_i)}) = \sqrt{1-q} \ket{1}\ket{\phi_1(\psi_i)} - \sqrt{q} \ket{0}\ket{\phi_0(\psi_i)}
\end{align*}
and acts trivially on the complement of the space spanned by $\{\ket{0}\ket{\phi_0(\psi_i)}\}\cup \{\ket{1}\ket{\phi_1 (\psi_i)}\}$.

Now we can define a unitary $Q = VU$, which we will argue is close to $U$ and moreover for every $\ket{\psi} \in \mathcal{H}$, $\ket{\psi}$ is an eigenvector of the following operator, 
\begin{align}\label{eq:projection_P}
P_1 = (\Id \otimes \bra{0})^{\dagger} Q^{\dagger} \Pi_1 Q (\Id \otimes \ket{0})
\end{align}
with the fixed eigenvalue ${q}$. In other words, $Q$ can be seen as a \emph{correction} of $U$. Now using lemma~\ref{lemma:success_prob}, by setting $q = \frac{1}{2^m}$ we have that, for some negligible function $\mu$, for all $\psi \in \mathcal{H}$, $|p(\psi)-q| \leq \mu(\lambda)$. Hence, we can bound the operator distance between $Q$ and $U$ by, 
\begin{align}
    |Q-U| = |(V - \Id)U|&\leq \max_{i \in [1,\dots,k]}\sqrt{(\sqrt{p(\psi_i)} - \sqrt{q})^2 + (\sqrt{1-p(\psi_i)} - \sqrt{1-q})^2 }\nonumber\\
    &\leq \sqrt{2\mu (\lambda)} = \negl(\lambda)\label{eq:Q_V_distance}
\end{align}

The trick is to replicate the proof of the quantum rewinding lemma from~\cite{DBLP:journals/siamcomp/Watrous09} with the projections $\Pi$ and $\Delta$, but with the unitary $Q$ instead of $U$. To do this, the adversary will compute the unitary $V$ and apply $VU$ when performing the alternation. One might notice that it might not be possible to compute $V$ exactly. In reality, $\adv$ will compute another unitary $\tilde{V}$ which is extremely close to $V$, and instead use $\tilde{Q} = \tilde{V}U$ in the process. However, as $\adv$ is computationally unbounded, they can estimate $V$ with very high precision, say find $\tilde{V}$ which is doubly inverse exponentially close to $V$. We will return to this matter at the end of the proof, but for now, let us assume $\adv$ is given the unitary $Q = VU$. 

Given $\Pi,\Delta$ and the unitary $Q$, and starting from the state $\ket{\psi} = \ket{pk}^{\otimes m}$ the adversary performs the following algoirthm. 

\medskip\noindent \underline{\textsf{get\_state}$(\psi , \Pi , \Delta , Q,q,\delta)$}:
\begin{itemize}
    \item Set  $t = 0$.
    \item Apply $Q$ on $\ket{\psi}\ket{0}$.
    \item While $t \leq \log(1/\delta)/(4q(1-q))$:
    \begin{itemize}
        \item Measure $\text{out}$ in computational basis.
        \item If the output is $1$, return the residual state $\ket{\psi_{fin}}$.
        \item Else if the output is $0$:
        \begin{itemize}
            \item Apply $Q^{\dagger}$ to the remaining state.
\item Perform a phase flip depending on output of $\Delta$, i.e. apply $2\Delta_0 - \Id$.
\item Apply $Q$ to the resulting state.
\item Set $t = t+1$.
        \end{itemize}
    \end{itemize}
    \item Return the residual state.
\end{itemize}
% \begin{figure}
% \noindent \underline{\textsf{get\_state}$(\psi , \Pi , \Delta , Q,q,\delta)$}
% \begin{algorithmic}[1]
% \State $t = 0$
% \State Apply $Q$ on $\psi$
% \While{$t \leq \log(1/\delta)/(4q(1-q))$}
% \State Measure $\text{out}$ in computational basis.
% \If{the measurement output is $1$}
% \State \Return the remaining state $\psi_{fin}$
% \EndIf
% \If{the measurement output is $0$} 
% \State Apply $Q^{\dagger}$ to the remaining state
% \State Perform a phase flip depending on output of $\Delta$, i.e. apply $2\Delta_0 - \Id$
% \State Apply $Q$ to the resulting state 
% \EndIf
% \EndWhile
% \State \Return the remaining state 
% \end{algorithmic}
% \caption{The rewinding procedure that with a high probability, on input state $\ket{\psi}\ket{0}$ returns $\Pi_1 Q \ket{\psi}\ket{0}$}
% \label{alg:alternate}
% \end{figure}
We prove that with probability $1-\delta$ the state outputted by the procedure is $\Pi_1 Q \ket{\psi}\ket{0}$. First we prove the claim that every $\ket{\psi} \in \mathcal{H}$ is an eigenvector of $P_1$, defined in equation~\ref{eq:projection_P} and $P_0 = \Id - P_1$ with corresponding eigenvalues ${q}$ and ${1-q}$. This is true as for each $i$ we have that, 
\begin{align*}
 \bra{\psi_i}(\Id \otimes \bra{0}) Q^{\dagger} \Pi_1 Q (1\otimes \ket{0})\ket{\psi_i} = \bra{0}\bra{\psi_i} U^{\dagger}V^{\dagger}\Pi_1 VU \ket{\psi_i}\ket{0} \\ 
 =\bra{0}\bra{\psi_i} U^\dagger V^\dagger \Pi_1 (\sqrt{q} \ket{1}\ket{\phi_1(\psi_i)} + \sqrt{1-q}\ket{0}\ket{\phi_0(\psi_i)}) \\ 
 = (\sqrt{q}\bra{\phi_1(\psi_i)}\bra{1} + \sqrt{1-q}\bra{\phi_0(\psi_i)}\bra{0}) (\sqrt{q} \ket{1} \ket{\phi_1(\psi_i)} ) \\= q
\end{align*}
As an operator $O$ can be uniquely determined by the parity function $\ket{\psi} \to \bra{\psi}O \ket{\psi}$, we deduce that $P_1$ ($P_0$ respectively) act as $q\times \Id$ ($(1-q)\times \Id$ respectively) on $\mathcal{H}$. As a result we have that, 
\begin{align}
    \Delta_0 Q^\dagger \Pi_1 Q \Delta_0 = (\Id \otimes \ket{0}) P_1 (\Id \otimes \bra{0}) = q\times \Delta_0 \label{eq:delta_action}
\end{align}
and similarly $\Delta_0 Q^\dagger \Pi_0 Q \Delta_0 = (1-q)\times \Delta_0$. Now let us iterate what will happen to the state throughout the procedure. After applying the unitary $Q$ on the state $\psi$ the state in hand would be the following, 
$$Q\ket{\psi}\ket{0} = \sqrt{q}\ket{1}\ket{\phi_1(\psi)}+ \sqrt{1-q}\ket{0}\ket{\phi_0(\psi)}$$

In case measuring $\Pi$ yields outcome $1$ we end up with the state $\ket{1}\ket{\phi_1(\psi)}$ which is exactly as desired. So let us assume the outcome is $0$. Now applying $Q^\dagger$, $2\Delta_0 - \Id$ and $Q$ consecutively we are left with the state 
\begin{align}
Q(2\Delta-1) Q^\dagger \ket{0}\ket{\phi_0(\psi)} &= \frac{1}{\sqrt{1-q}}Q(2\Delta_0 - 1) \Pi_0 Q\Delta_0 \ket{\psi}\ket{0}\label{eq:state_trans_mv1}\\
& = 2\sqrt{1-q} Q\ket{\psi}\ket{0} - \frac{1}{\sqrt{1-q}}\Pi_0 Q\ket{\psi}\ket{0} \label{eq:state_trans_mv2}\\ 
& = 2\sqrt{q(1-q)}\ket{1}\ket{\phi_1(\psi)} + (1-2q)\ket{1}\ket{\phi_0(\psi)}\label{eq:state_trans_mw}
\end{align}
Where the transition from equation~\ref{eq:state_trans_mv1} to \ref{eq:state_trans_mv2} is due to equation~\ref{eq:delta_action}. What matters, is that this vector is still in the two dimensional space spanned by $\ket{0}\ket{\phi_0(\psi)}$ and $\ket{1}\ket{\phi_1(\psi)}$ and measuring it with respect to $\Pi$ yields outcome $1$ and residual state $\ket{1}\ket{\phi_1(\psi)}$ with probability $4 p (1-p)$ and outcome $0$ and state $\ket{0}\ket{\phi_0(\psi)}$ with probability $(1-2q)^2$. Notice that if measuring $\Pi$ yields output $0$ again, the residual state would be $\ket{0}\ket{\phi_0(\psi)}$ and the state at the beginning of the next round would again be as described in equation~\ref{eq:state_trans_mw}. Hence the probability of the procedure not outputting $1$ after $t+1$ repetitions is given by $(1-q)(1-2q)^{2t}$. Hence by setting $t = O(\log(1/\delta)\frac{1}{q(q-1)})$, this probability would be less than $\delta$. 

This allows us to conclude that with probability $1-\delta$, the adversary would have the state $\Pi_1 Q \ket{pk}^{\otimes}\ket{0}$ after running the procedure, which combined with equation~\ref{eq:Q_V_distance}, shows that they have a state negligibly close to $\Pi_1 U \ket{pk}^{\otimes m}\ket{0}$. This allows us to invoke lemma~\ref{lemma:output_state} which implies applying the unitary $U_{enc}^{\dagger}U_{dec}^{\dagger}U_{comp}^{\dagger}$ on the adversaries state, would leave the state at negligible distance from the state $\ket{\tilde{\psi}}$,
\begin{align}
    \ket{\tilde{\psi}} = \ket{pk}^{\otimes m}\sum_{b_1,\dots,b_m} \ket{b_1\dots b_m}_b\sum_{sk\in S_{1/\log(m)}}\ket{sk}_{sk}\ket{0}
\end{align}
where $S_{1/\log(m)}=\{sk| Pr_{b\sim U}[Dec(sk,Enc(pk,b)) = b]\geq 1-1/\log(m)\}$. All left to do for $\adv$ is to measure the $sk$ register to recover a secret key $sk^*$ on this state and on a challenge ciphertext ${ct}^*$, return $Dec(sk^*,{ct}^*)$. Due to the definition of $S_{\log(m)}$ the probability of $\adv$ decrypting $\hat{ct}$ correctly is $(1-\delta - \negl(\lambda))(1-\frac{1}{\log(m)})$. By setting $\delta \approx 1/2^{m}$, the probability of decrypting correctly would be significantly more than $1/2$. 

\noindent\textbf{Realizing unitary $V$}:\\
The only subtlety left is realizing the unitary $V$. We will explicitly use the fact that $\adv$ is computationally unbounded. Note that any unitary operator can be approximated to arbitrary accuracy with \textsf{CNOT}, Hadamard, phase and $\pi/8$ gates~\cite[Chapter 4.5]{DBLP:books/daglib/0046438}. Hence there exists a quantum circuit $C$, most likely inefficient, such that $C$ computes a unitary $\tilde{V}$ such that $|\tilde{V} - V| \leq O(2^{-2^{\lambda}})$, i.e. $\tilde{V}$ is doubly exponentially close to $V$. 

This would also imply that $\tilde{Q} = \tilde{V}U$ is $O(2^{-2^{\lambda}})$ close to $Q$ in operator distance. Hence, we can consider $\adv$ to be a non-uniform adversary who is given the description of the circuit $C$. Note that the description of $C$ is only dependent on $U$, hence independent of the challenge public keys and ciphertext. So in reality $\adv$ will run the \textsf{get\_state} procedure with the unitary $\tilde{Q}$ instead of $Q$ and we prove that the output of the process is in fact negligibly close to $\Pi_1 Q\ket{pk}^{\otimes m}\ket{0}$, hence negligibly close to the desired state $\Pi_1 U\ket{pk}^{\otimes m}\ket{0}$. This is done similarly to the proof of perturbed version of the quantum rewinding lemma from~\cite{DBLP:journals/siamcomp/Watrous09}. 

We bound the distance of the output of the procedure ran with $\tilde{Q}$ and $\Pi_1 Q\ket{pk}^{\otimes m}\ket{0}$ using triangle inequality. At each iteration, the distance between the states, when running the algorithm with $\tilde{Q}$ or with $Q$ is bounded by $|\tilde{Q}-Q| = O(2^{-2^{\lambda}})$. To elaborate, let us call the states after the first iteration $\ket{\phi}$ and $\ket{\phi'}$. Now we have that $d(\ket{\phi} , \ket{\phi'})\leq O(2^{-2^{\lambda}})$, and we wish to bound the distance between $\tilde{Q}\ket{\phi}$ and $Q\ket{\phi'}$. This can be done as follows, 
\begin{align*}
    |Q\ket{\phi'} - \tilde{Q}\ket{\phi}| \leq |Q(\ket{\phi'}- \ket{\phi})|+ |(Q-\tilde{Q})\ket{\phi}|= O(2^{-2^{\lambda}})
\end{align*}
Where the first inequality follows from triangle inequality and the second from the distance bounds given in the previous paragraph. With the same argument we can show that at each iteration the distance increases at most by $|Q-\tilde{Q}|$, hence by $O(2^{-2^{\lambda}})$. Hence after $t = O(\frac{1}{q(q-1)})$ iterations the distance would increase by $O(2^{\textsf{poly}(\lambda)})\times O(2^{-2^{\lambda}})$ which is still negligible in $\lambda$. This concludes the proof of Theorem~\ref{thm:impossibility}.

\qed
\end{proof} 

==> overview_impossibility.tex <==
% !TEX root = main.tex
Next we turn to the second and technically more involved contribution of this paper, where we show that computational assumptions are necessary to constructing a quantum PKE.
As a warm-up, let us discuss a few possible strategy to show that \emph{classical} PKE is impossible unconditionally.
This is of course an easy exercise, but is illustrative to see what goes wrong in the setting where public keys are allowed to be quantum.

The first approach would be to try to invert the key generation algorithm. More specifically, a  computationally unbounded adversary can iterate through all possible choices of randomness~$r$ in the key generation algorithm and check whether the public key generated with randomness~$r$ matches the challenge public key~$\pk$.
Later, the adversary could use the secret key generated by~$r$ to decrypt the challenge ciphertext.
The issue with generalizing this approach to the quantum setting is that when the public keys are quantum, checking whether the derived public key and the challenge one are the same is less immediate.
One natural idea is to use a SWAP test~\cite{buhrman2001quantum} to compare the two public keys, but note that each time a SWAP test is performed the challenge public key will be disturbed by some amount.
Since on average an exponential number of SWAP tests need to be performed, this would mean that the challenge public key will be significantly disturbed before the adversary has found the correct configuration of randomness.

\subsubsection{Warm-Up Solution: Classical Ciphertexts.}
The second method consists of an adversary picking $m$ random plaintexts, encrypting them all with respect to $\pk$ to obtaint the ciphertexts  $\ct_1,\dots,\ct_m$,  and iterate through all possible values of $\sk$ until they find one which decrypts all $m$ ciphertexts correctly. It turns out that this approach is more promising, and we can in fact show that this argument can be made to work, however only in the \emph{simplified settings} where we assume that all ciphertexts are classical.\footnote{Although in our actual scheme the ciphertexts are indeed classical, we want to rule out the general case, where ciphertexts may be quantum states.}
We describe an unbounded adversary $\adv$ which wins the IND-CPA game with a non-negligible advantage. For convenience, we assume that the scheme has perfect correctness, but the argument can be extended to schemes with imperfect correctness as well. For a polynomial $m$, given $m$ copies of the public key $pk$ they act as follows.

\medskip\noindent
\underline{$\adv(\pk^{m(\lambda)} , \ct)$:}
\begin{itemize}
    \item Pick $m(\lambda)$ plaintexts $\pt_0,\dots,\pt_{m-1}$ uniformly at random.
    \item For $i\in \{0,\dots,m-1\}$: Compute $\ct_i \gets \Enc(\pk , \pt_i)$.
    \item Enter the following loop:
    \begin{itemize}
        \item Pick $\sk^*$ uniformly at random from the domain of the secret keys.
        \item For $i\in \{0,\dots,m-1\}$: Compute ${\pt_i}^* \gets \Dec(\sk^* , \ct_i)$.
        \item If there exists some $i$ such that $\pt_i^* \neq \pk_i$ then restart the loop. Else exit.
    \end{itemize}
    \item Let $\sk^*$ be the key selected by the above procedure. Use $\sk^*$ to decrypt the challenge ciphertext.
\end{itemize}
Note that, we implicitly use the fact that the ciphertext is classical, as we use the same ciphertext for each guess of $sk$, i.e.~we are copying the ciphertext exponentially many times. Also note that eventually the algorithm will exit the loop, since there exists at least one secret key with perfect correctness. So what is left to be shown is that the secret key output by this procedure is good, in the sense that it has an overall good success probability. More formally,
let us define $p_{\sk^*}$ to be
\begin{align*}
    p_{\sk^*} = Pr_{\ct} [\Dec(\sk^*, \ct) = \Dec(\sk,\ct)]
\end{align*}
i.e.~the probability of $\sk^*$ decrypting a uniformly random ciphertext correctly. Fix any particular $\sk^*$ such that $p_{\sk^*} \leq 3/4$, then the probability that the all of the ciphertexts will decrypt correctly is
\[
p_{\sk^*}^{m} = \left(\frac{3}{4}\right)^m.
\]
Thus, for a large enough $m$, the key output by the above procedure will have success probability greater than 3/4 with all but negligible probability, by a union bound.






% %HERE
% Note that proving the impossibility of an unconditionally secure classical PKE is rather trivial and we believe a good way to explain the challenges of proving a similar statement for quantum PKEs is to see what would go wrong if one tries to emulate the same proof for the quantum case.

% There are two generic ways to break the CPA security of any claimed unconditionally secure classical PKE. The first is by inverting the key generation algorithm. More precisely, a computationally unbounded adversary can iterate through all possible choices of randomness in the key generation algorithm $r$ and check whether the public-key generated with randomness $r$ matches the challenge public key $\pk$. Later the adversary could use the secret key generated by $r$ to decrypt the challenge ciphertexts.


% Now let us see the issues that occur in each approach when we have public-keys that are quantum states. The issue with the first approach is that one can not check whether the public-key generated by randomness $r$ is actually matching the challenge public-key. One could in fact, try to swap test the derived public-key and the challenge one, however, each time a swap test is performed the challenge public-key will be disturbed by some amount. Note that on average exponential number of swap tests are required which would mean with a high probability, the challenge public-key will be significantly disturbed before the adversary has found the correct configuration of randomness.

% To demonstrate the issues with the second approach we first provide a proof for a weaker version of the theorem in which in fact a very similar approach can be employed. Namely, we prove the impossibility in the case where the ciphertexts are classical bit strings.
% % Let us see how emulating the generic proof for the impossibility of unconditionally secure classical PKE works out in this setting. Classically an unbounded adversary returns $(\pt_0,\pt_1)$ to the game and is given $\ct$ which is the encryption of one of the two plaintexts at random, and their goal is to determine which message was encrypted. The adversary can do the following,
% % \begin{enumerate}
% %     \item Pick a large number $m$
% %     \item Pick $m$ random messages $\pt_1,\dots,\pt_m$
% %     \item Pick a secret-key guess $\sk$
% %     \item Encrypt $\pt_i$ and decrypt with the secret-key guess $\sk$.
% %     \item If all the decryptions match the original plaintexts use this key guess to decrypt the challenge $\ct$
% % \end{enumerate}
% % Why can not we use the same argument for the quantum PKE? The caveat is that in the quantum PKE setting each time an encryption has been done, one public-key is consumed. Note that the procedure should be repeated $\Theta(2^{\poly(\lambda)})$ times hence the naive approach would require an exponential number of public-keys which is not provided to the adversary by the security game.

% % This problem is easy to fix when the public-keys are quantum states but ciphertexts are considered to be classical bit-strings. Let us elaborate.
% \begin{theorem}\label{thm:impossibility_light}
% For any quantum PKE, $\Gamma$, with classical ciphertext and perfect correctness, there exists a quantum algorithm $\adv$, that wins the $\indcpa$ game with a probability significantly more than $1/2$.
% \end{theorem}
% \begin{proof}[Proof Sketch]
% We describe an unbounded adversary $\adv$ which wins the IND-CPA game with a non-negligible advantage. For convenience, we assume that the scheme has perfect correctness, but the argument can be extended to schemes with imperfect correctness as well. For a polynomial $m$, given $m$ copies of the public key $pk$ they act as follows.

% \medskip\noindent
% \underline{$\adv(\pk^{m(\lambda)} , \ct)$:}
% \begin{itemize}
%     \item Pick $m(\lambda)$ plaintexts $\pt_0,\dots,\pt_{m-1}$ uniformly at random.
%     \item For $i\in \{0,\dots,m-1\}$: Compute $\ct_i \gets \Enc(\pk , \pt_i)$.
%     \item Enter the following loop:
%     \begin{itemize}
%         \item Pick $\sk^*$ uniformly at random from the domain of the secret keys.
%         \item For $i\in \{0,\dots,m-1\}$: Compute ${\pt_i}^* \gets \Dec(\sk^* , \ct_i)$.
%         \item If there exists some $i$ such that $\pt_i^* \neq \pk_i$ then restart the loop. Else exit.
%     \end{itemize}
%     \item Let $\sk^*$ be the key selected by the above procedure. Use $\sk^*$ to decrypt the challenge ciphertext.
% \end{itemize}
% % \begin{algorithmic}[1]
% % \State Pick $m(\lambda)$ plaintexts $\pt_0,\dots,\pt_{m-1}$ uniformly at random
% % \For{$i \in \{0,\dots,m-1\}$}
% % \State $\ct_i \gets Enc(pk , \pt_i)$
% % \EndFor
% % \While{\textsf{True}}
% % \State pick $\sk^*$ uniformly at random from the domain of secret keys
% % \State $\textsf{bool} \gets \textsf{True}$
% % \For{$ i \in \{0,\dots,m(\lambda)\}$}
% %     \State $\widetilde{\pt_i} \gets \Dec(\sk^* , \ct_i)$
% %     \If{$\widetilde{\pt_i}\neq \pt_i$}
% %     \State \textsf{bool}$\gets$\textsf{False}
% %     \EndIf
% % \EndFor
% % \If{\textsf{bool} $= \textsf{True}$}
% % \State \Return $\tilde{b} \gets \Dec(\sk^*,ct)$
% % \EndIf
% % \EndWhile
% % \State \Return $\bot$
% % \end{algorithmic}
% Note that, we implicitly use the fact that the ciphertext is classical, as we use the same ciphertext for each guess of $sk$, i.e.~we are copying the ciphertext exponentially many times. Also note that eventually the algorithm will exit the loop, since there exists at least one secret key with perfect correctness. So what is left to be shown is that the secret key output by this procedure is good, in the sense that it has an overall good success probability. More formally,
% let us define $p_{\sk^*}$ to be
% \begin{align*}
%     p_{\sk^*} = Pr_{\ct} [\Dec(\sk^*, \ct) = \Dec(\sk,\ct)]
% \end{align*}
% i.e.~the probability of $\sk^*$ decrypting a uniformly random ciphertext correctly. Fix any particular $\sk^*$ such that $p_{\sk^*} \leq 3/4$, then the probability that the all of the ciphertexts will decrypt correctly is
% \[
% p_{\sk^*}^{m} = \left(\frac{3}{4}\right)^m.
% \]
% Thus, for a large enough $m$, the key output by the above procedure will have success probability greater than 3/4 with all but negligible probability, by a union bound. This concludes our proof.

% \end{proof}
% \begin{remark}
% As a side remark, the above argument can be extended to the case of imperfect correctness. Let us say the correctness error is $\epsilon$. The trick would be to set a threshold $1-\epsilon'$, for some $\epsilon' < \epsilon$, and check whether at least $(1-\epsilon')m$ ciphertexts decrypted correctly. Then one can use Chernoff bounds to determine how many times the experiment should be ran to make sure with high probability the error in estimating the success probability of a guessed secret key is less than $\epsilon - \epsilon'$.
% \end{remark}

\subsubsection{The General Case}
As already alluded to earlier, one immediate obstable for the general case (when the ciphertexts are also allowed to be quantum states) is that the above adversary heavily relies on being able to reuse the $m$ ciphertexts they prepare at the beginning of the procedure. However, if the ciphertexts are also quantum states the no-cloning theorem would prevent this. To circumvent this, the natural idea would be to take a purification approach. Meaning, we would defer the operations that would cause a disturbance to the states, i.e. measurements, and instead only perform a single qubit measurement which would just indicate if the process succeeds in the current iteration.

% \subsubsection{Purification strategy}
% In the case when the ciphertexts are also allowed to be quantum states, the problem is significantly more challenging. For instance, note that the proof of \cref{thm:impossibility_light} heavily relied on the adversary copying the ciphertexts as many times they please. However, when the ciphertexts are also quantum states, one can copy the ciphertexts no more.

% Note that the only operations that irreversibly damage the public-key copies
% are measurements, hence a natural direction would be to take a purification approach. Meaning we would defer the measurements to the last iteration, and at each loop only apply a single qubit gentle measurement which the outcome indicates whether the procedure will succeed or not.

 More precisely, we consider an adversary that starts with $m$ copies of the public-key $\ket{\psi} = \ket{\pk}^{\otimes m}$, and applies a unitary $U$ on $\ket{\psi}\ket{0}$ which does a purified version of the following task:
 \begin{enumerate}
     \item Loads $m$ uniform plaintexts $b_1,\dots,b_m$ and a uniformly random secret-key $\sk$ on the ancilla registers.
     \item Encrypts the $m$ plaintexts with respect to $\ket{\pk}$.
     \item Decrypts the $m$ ciphertexts with respect to $\sk$.
     \item Loads $1$ into an output register ``$\out$'' if all the ciphertexts decrypted correctly.
 \end{enumerate}
 If we let $\Pi_1 = \ket{1}\bra{1}_{\out}\otimes \id$ the goal would be to find a procedure that terminates with the state $\Pi_1 U \ket{\psi}\ket{0}$. One might notice that $\bra{\psi} U^{\dagger}\Pi_1 U\ket{\psi} \approx 1/2^m$, hence a naive approach would be to bound how much the state would be disturbed by the operator $U^{\dagger}(\id - \Pi_1)U$ using the gentle measurement lemma~\cite[Lemma 9]{DBLP:journals/tit/Winter99}. However, a more careful look shows that after $t$ iterations of the procedure failing, i.e.~measuring $\Pi$ yielding $0$, the guarantee is that the distance of the state from the original is bounded by $(\frac{1}{2^m})^{1/2^t}$. This exponential distance growth means that it is hard to argue about the closeness of the residual state from the original only after a polynomially many iterations, and it is quite evident that the number of iterations required for the procedure to succeed is $O(2^m)$.

 \subsubsection{Quantum Rewinding via Alternating Projectors.} Our idea to bypass the above obstacle is to use the quantum rewinding lemma from Watrous~\cite{DBLP:journals/siamcomp/Watrous09}. This idea has been used before to provide tighter bounds than the ones provided by the gentle measurement lemma, so it is plausible to expect that it would be useful also in our context. Unfortunately it turns out that a naive application of the quantum rewinding lemma is \emph{still} not sufficient in our use case.

 On a high level, the (perturbed) quantum rewinding lemma states that for a unitary $U$ and a rank-one projective measurement $\{\Pi_1,\id -\Pi_1\}$, if constants $q$ and $\epsilon$ exist such that for all $\ket{\psi}$, $\bra{\psi}U^\dagger \Pi_1U \ket{\psi} \in [q -\epsilon , q+\epsilon]$, for each $\delta\in (0,1)$ a procedure $C$ exists that satisfies the following two properties:
 \begin{itemize}
     \item $C$ terminates in time $T = O(\frac{1}{q}\log(1/\delta)\text{size}(U))$.
     \item With probability at least $1-\delta$, the residual state of $C$ is in at most $O(\log(1/\delta) \frac{1}{q}\epsilon)$ distance from $\Pi_1 U \ket{\psi}\ket{0}$.
 \end{itemize}
 A careful look at the statement makes it evident that the lemma can not be of use when $1/q$ is exponentially large, as even if $\epsilon$ is a negligible function the lemma does not guarantee that the final state would be close to the desired one as $O(\frac{1}{q}\epsilon)$ might still be significantly large.

 \subsubsection{The Unbounded Quantum Rewinding Lemma.} This brings us to the main technical contribution of this work. We observe that for our lower bound we do not need the procedure to be efficient, rather just the final state to be close to the desired one. Hence, we prove a new version of the quantum rewinding lemma, altered as follows: Let $U$ and $\Pi_1$ be as before and let $q$ exist such that for all $\ket{\psi}$, $\bra{\psi}U^\dagger \Pi_1 U\ket{\psi} \in [q -\negl , q+\negl]$, then for all $\delta\in (0,1)$ there exists a procedure $C$ such that:
 \begin{itemize}
     \item $C$ terminates.
     \item With probability $1-\delta$, the residual state of $C$ is in negligible distance from $\Pi_1U\ket{\psi}\ket{0}$.
 \end{itemize}
 Note that, although this lemma only guarantees that $C$ terminates, the distance guarantee is the only property required for our impossibility result. Let us briefly give an intuition of how this lemma can be proven. The idea of the proof is to make $C$ implement a \emph{correction} unitary. Meaning, a unitary $V$ such that letting $Q = VU$, there exists a constant $Q$ such that for all $\ket{\psi}$, $\bra{\psi}Q^\dagger \Pi_1 Q\ket{\psi} = q$. Note that $V$ would be very close to the identity as the spectrum of $U\Pi_1U$ is already concentrated around $q$ and each value has to be changed by a negligible amount.

 Now one can imagine running the non-perturbed version of the quantum rewinding lemma for $Q$ instead of $U$. This would guarantee that, with a high probability, the procedure terminates with the state $Q\Pi_1\ket{\psi}\ket{0}$ which, as $V$ is close to identity, is extremely close to $U\Pi_1\ket{\psi}\ket{0}$. We discuss in detail how such a \emph{correction} unitary can be realized in \cref{sec:generic_rewinding_lemma} but to put it short, instead of realizing $V$, the procedure implements an approximation of it with enough precision that the output state would still be in negligible distance of the desired state.
 % $m$ uniformly picked bits $b_1,\dots,b_m$, and a uniformly selected secret key guess $\sk$. The adversary later proceeds by applying a unitary which encrypts the $m$ messages using $\pk$, decrypts the obtained ciphertexts with $\sk$ and loads $1$ unto an ancilla register, called the \emph{output} register, if all the decrypted values match the originally picked plaintexts. Note that although encryption and decryption might contain measurements, here we consider a purified version of the operator in which the measurements are replaced with CNOTing the measured wire to some ancilla register.

% Now the adversary can measure the \emph{output} register which would indicate whether all plaintexts were decrypted correctly or not. As on average over $\sk$ the probability of this measurement outputting $1$ is negligible, we can deduce that this is a gentle measurement that would not disturb the original state by much.

% The natural approach would be to bound this disturbance using the gentle measurement lemma~\cite{DBLP:journals/tit/Winter99}. However, the gentle measurement lemma would only guarantee, the error after each failed loop is at most the square root of the already existing error. This would mean the error would become noticeable after only polynomially many repetitions of the loop.

% This impairs the use of this strategy as the adversary in our case would need to repeat the procedure for the majority of the key space, i.e. exponentially many times. This indicates that a tighter rewinding technique is required.

% \subsubsection{Quantum Rewinding Lemma.} The alternative approach to achieve a tighter error propagation is using the quantum rewinding Lemma~\cite{DBLP:journals/siamcomp/Watrous09}. Let us go over the strategy and issues that arise. We start with the following state:
% $$\ket{\psi} = \sum_{\sk,b} \ket{\pk}^{\otimes m}\ket{\sk}\ket{b_1,\dots,b_m}\ket{0}$$
% We also consider a similar unitary as we described in the previous approach, i.e. a unitary that encrypts $b_1,\dots,b_m$ with $\pk$, decrypts them with respect to $\sk$ and loads $1$ unto an ancilla qubit, named \emph{output} register, if all the ciphertexts decrypt correctly to their original plaintexts.

% Now consider a projective measurement $\{\Pi_1 = \ket{1}\bra{1}_{\text{\emph{output}}}\otimes \id , \id-\Pi_1\}$. Our goal is to be left with the state $\Pi_1 U \ket{\psi}$, i.e. the subspace in which $m$ uniform plaintexts decrypted correctly with respect to a key $\sk$. This formalization makes the problem suit the quantum rewinding lemma framework quite well. However, there are still issues.

% First of all, applying the rewinding lemma would require that probability of obtaining $1$ when measuring $\{\Pi_1, \id - \Pi_1\}$ is the same for all $\psi$. This is not the case for us, for instance, one might consider a PKE that for a negligible fraction of the public key space, most secret keys decrypt messages correctly. This can be resolved by using a perturbed version of the rewinding lemma which only requires that the probability of measuring $1$ would be concentrated around a constant $q$ with the maximum distance $\delta$.

% In fact, we can show that in our case, for every honestly generated public-key, the probability of measuring $1$ after applying $U$ and measuring $\Pi$ is in negligible distance from a constant. However, there is another issue that we run into. The problem again arises from rewinding the process exponentially many times, as the perturbed quantum rewinding lemma only guarantees that if the process was run $T$ times, the final state is in $T\delta$ distance from the desired state, i.e. $\Pi_1U\ket{\psi}$.

% Although $\delta$ is negligible in $\lambda$, as $T$ is exponential, a naive application of Watrous' rewinding lemma would not be sufficient in our case.
% \subsubsection{The correction Unitary}
% This brings us to the main technical contribution of this work. We prove an altered version of Watrous' quantum rewinding lemma which allows us to rewind the procedure exponentially many times without accumulating an additive error. Note that for our purpose, we do not require any bounds on the complexity of the rewinding procedure, but just for it to terminate.

% Let us elaborate on the proof technique. Note that as we mentioned for all $\ket{\pk}$, the probability of measuring $\Pi$ returning $1$, after $U$ is applied is in negligible distance from a constant $q$. So what if we could realize a unitary $V$, such that for $Q = VU$ this probability is not in negligible distance from $q$ but exactly $q$? In a sense, $V$ can be seen as a correction unitary, which fixes the spectrum of an operator defined by $U$ and $\Pi$.

% As it turns out such unitary does exist, however, it might not be possible to implement exactly. Here we make use of a universality theorem to say although $V$ might not be implementable, we can approximate it with a universal gate set up to any desired precision, for instance, $\delta$ such that $2^m \delta$ is still negligible. To finish off the proof, we just perform Watrous' rewinding procedure to find $\Pi_1 VU\ket{\psi}$ instead which we argue is negligibly close $\Pi_1 U\ket{\psi}$ because $V$ is extremely close to the identity.


==> pke_prfs.tex <==
% !TEX root = main.tex
\underline{\textsf{key\_gen}}
\begin{enumerate}
    \item Pick two PRFS keys $k_0$ and $k_1$
    \item Prepare the state $\ket{pk} = \sum_{x}\ket{x}_X\ket{\text{PRFS}_{x,k_1}}\ket{\text{PRFS}_{x,k_2}}$
\end{enumerate}
\underline{\textsf{Enc(b)}}
\begin{enumerate}
    \item Measure the $X$ register of $\ket{pk}$ to obtain $x$ and the states $\ket{x}\otimes \ket{\psi_1}\otimes \ket{\psi_2}$. 
    \item Prepare the state $\ket{ct} = 1/\sqrt{2}(\ket{0}\ket{\psi_1} + (-1)^b\ket{1}\ket{\psi_2})$
    \item Return $x ,\ket{ct}$ as the ciphertext
\end{enumerate}
\underline{\textsf{Dec}}
\begin{enumerate}
    \item Uncompute $\ket{\psi_1}$ and $\ket{\psi_2}$ controlled on the first qubit
    \item Measure the first qubit in Hadamard Basis
\end{enumerate}


==> proof_rewinding_lemma.tex <==
% !TEX root = main.tex
\begin{proof}[\cref{lemma:generic_rewinding_lemma}]
The goal is to define a process which for all $\ket{\psi}\in \mathcal{H}$, starting with the state $\ket{\psi}\ket{0}_{aux}$, outputs the state $\Pi_1 U\ket{\psi}\ket{0}_{aux}$. The idea is to follow a similar approach to the quantum rewinding lemma proof from~\cite{DBLP:journals/siamcomp/Watrous09}. We define $\Delta = \{\Delta_0 ,\Id - \Delta_0\}$ to be a projective measurement such that $\Delta_0 =\Id \otimes \ket{0}\bra{0}_{aux}$, i.e. a projection unto the space where all auxiliary qubits are set to $0$. 

Following the notation used in \cref{lemma:orthonormal_basis}, for all $\ket{\psi}\in \mathcal{H}$ we define, $\phi_0(\psi)$, $\phi_1(\psi)$ and $p(\psi)$ to be the unique vectors and values such that, 
\begin{align*}
    U \ket{\psi}\ket{0} = \sqrt{p(\psi)}\ket{1}_{\text{out}}\ket{\phi_1(\psi)} + \sqrt{1-p(\psi)}\ket{0}_{\text{out}}\ket{\phi_0(\psi)} 
\end{align*}

We further define $\{\psi_i\}_{i \in [1,\dots,k]}$ to be the orthonormal basis of $\mathcal{H}$ induced by the eigenvectors of the operator
$$P = (\Id \otimes \bra{0})^{\dagger} U^{\dagger} \Pi_1 U (\Id \otimes \ket{0})$$
Now due to \cref{lemma:orthonormal_basis} we have that $\{\ket{0}\ket{\phi_0(\psi_i)}\}\cup \{\ket{1}\ket{\phi_1 (\psi_i)}\}$ forms an orthonormal basis for the support of $U (\Id\otimes \ket{0})$. This allows us to define a unitary $V$ which acts as follows, 
\begin{align*}
    V(\sqrt{p(\psi_i)} \ket{1}\ket{\phi_1(\psi_i)} + \sqrt{1-p(\psi_i)} \ket{0}\ket{\phi_0(\psi_i)}) = \sqrt{q} \ket{1}\ket{\phi_1(\psi_i)} + \sqrt{1-q} \ket{0}\ket{\phi_0(\psi_i)} \\
    V(\sqrt{1-p(\psi_i)} \ket{1}\ket{\phi_1(\psi_i)} - \sqrt{p(\psi_i)} \ket{0}\ket{\phi_0(\psi_i)}) = \sqrt{1-q} \ket{1}\ket{\phi_1(\psi_i)} - \sqrt{q} \ket{0}\ket{\phi_0(\psi_i)}
\end{align*}
and acts trivially on the complement of the space spanned by $\{\ket{0}\ket{\phi_0(\psi_i)}\}\cup \{\ket{1}\ket{\phi_1 (\psi_i)}\}$. This can be seen as a correction unitary, i.e. a unitary that fixes the spectrum of the operator $P$. 

We  define a unitary $Q = VU$, i.e. the correction of $U$. We later argue that $Q$ is close to $U$ but first let us elaborate on what we mean by \emph{correction}. The property of $Q$ that we are looking for is that for every $\ket{\psi} \in \mathcal{H}$, $\ket{\psi}$ is an eigenvector of the following operator, 
\begin{align}\label{eq:projection_P}
P_1 = (\Id \otimes \bra{0})^{\dagger} Q^{\dagger} \Pi_1 Q (\Id \otimes \ket{0})
\end{align}
with the fixed eigenvalue ${q}$. 

To prove $Q$ is in fact is close to $U$ we employ the condition that eigenvalues of $P$ are in a negligible distance of $q$. Let us compute the operator distance between $Q$ and $U$.  
\begin{align}
    |Q-U| = |(V - \Id)U|&\leq \max_{i \in [1,\dots,k]}\sqrt{(\sqrt{p(\psi_i)} - \sqrt{q})^2 + (\sqrt{1-p(\psi_i)} - \sqrt{1-q})^2 }\nonumber\\
    &\leq \sqrt{2\mu (\lambda)} = \negl(\lambda)\label{eq:Q_V_distance}
\end{align}
% \comm{KH}{change the neg to delta}
% The trick is to replicate the proof of the quantum rewinding lemma from~\cite{DBLP:journals/siamcomp/Watrous09} with the projections $\Pi$ and $\Delta$, but with the unitary $Q$ instead of $U$. To do this, the adversary will compute the unitary $V$ and apply $VU$ when performing the alternation. One might notice that it might not be possible to compute $V$ exactly. In reality, $\adv$ will compute another unitary $\tilde{V}$ which is extremely close to $V$, and instead use $\tilde{Q} = \tilde{V}U$ in the process. However, as $\adv$ is computationally unbounded, they can estimate $V$ with very high precision, say find $\tilde{V}$ which is doubly inverse exponentially close to $V$. We will return to this matter at the end of the proof, but for now, let us assume $\adv$ is given the unitary $Q = VU$. 
The original rewinding lemma uses the bound in \cref{eq:Q_V_distance} to bound the distance of the residual state from the desired state. Intuitively if $U$ was replaced with $Q$ each time the procedure is rewound and $U$ is applied, the outcomes of the two cases are negligibly close to one another. However, in our case, if we believe the process might be rewound exponentially many times, this additive error might end up being noticeable. 

The way to circumvent this is actually replacing $U$ with $Q$ in the rewinding procedure. This is equivalent to having a procedure which can implement the unitary $V$. Notice that this procedure is most probably not efficient, however efficiency is not a requirement of our lemma. We will discuss how $V$ can be implemented in detail towards the end of the proof but for now we assume the procedure is given an implementation of the unitary $V$, hence $Q = VU$.  

Given $\Pi,\Delta$ and the unitary $Q$, and starting from the state $\ket{\psi}\ket{0}^{\otimes m}$ the adversary performs the following algoirthm. 

\medskip\noindent \underline{\textsf{get\_state}$(\psi , \Pi , \Delta , Q,q,\delta)$}:
\begin{itemize}
    \item Set  $t = 0$.
    \item Apply $Q$ on $\ket{\psi}\ket{0}$.
    \item While $t \leq \log(1/\delta)/(4q(1-q))$:
    \begin{itemize}
        \item Measure $\text{out}$ in computational basis.
        \item If the output is $1$, return the residual state $\ket{\psi_{fin}}$.
        \item Else if the output is $0$:
        \begin{itemize}
            \item Apply $Q^{\dagger}$ to the remaining state.
\item Perform a phase flip depending on output of $\Delta$, i.e. apply $2\Delta_0 - \Id$.
\item Apply $Q$ to the resulting state.
\item Set $t = t+1$.
        \end{itemize}
    \end{itemize}
    \item Return the residual state.
\end{itemize}
% \begin{figure}
% \noindent \underline{\textsf{get\_state}$(\psi , \Pi , \Delta , Q,q,\delta)$}
% \begin{algorithmic}[1]
% \State $t = 0$
% \State Apply $Q$ on $\psi$
% \While{$t \leq \log(1/\delta)/(4q(1-q))$}
% \State Measure $\text{out}$ in computational basis.
% \If{the measurement output is $1$}
% \State \Return the remaining state $\psi_{fin}$
% \EndIf
% \If{the measurement output is $0$} 
% \State Apply $Q^{\dagger}$ to the remaining state
% \State Perform a phase flip depending on output of $\Delta$, i.e. apply $2\Delta_0 - \Id$
% \State Apply $Q$ to the resulting state 
% \EndIf
% \EndWhile
% \State \Return the remaining state 
% \end{algorithmic}
% \caption{The rewinding procedure that with a high probability, on input state $\ket{\psi}\ket{0}$ returns $\Pi_1 Q \ket{\psi}\ket{0}$}
% \label{alg:alternate}
% \end{figure}
We prove that with probability $1-\delta$ the state outputted by the procedure is $\Pi_1 Q \ket{\psi}\ket{0}$. First we prove the claim that every $\ket{\psi} \in \mathcal{H}$ is an eigenvector of $P_1$, defined in \cref{eq:projection_P} and $P_0 = \Id - P_1$ with corresponding eigenvalues ${q}$ and ${1-q}$. This is true as for each $i$ we have that, 
\begin{align*}
 \bra{\psi_i}(\Id \otimes \bra{0}) Q^{\dagger} \Pi_1 Q (1\otimes \ket{0})\ket{\psi_i} = \bra{0}\bra{\psi_i} U^{\dagger}V^{\dagger}\Pi_1 VU \ket{\psi_i}\ket{0} \\ 
 =\bra{0}\bra{\psi_i} U^\dagger V^\dagger \Pi_1 (\sqrt{q} \ket{1}\ket{\phi_1(\psi_i)} + \sqrt{1-q}\ket{0}\ket{\phi_0(\psi_i)}) \\ 
 = (\sqrt{q}\bra{\phi_1(\psi_i)}\bra{1} + \sqrt{1-q}\bra{\phi_0(\psi_i)}\bra{0}) (\sqrt{q} \ket{1} \ket{\phi_1(\psi_i)} ) \\= q
\end{align*}
As an operator $O$ can be uniquely determined by the parity function $\ket{\psi} \to \bra{\psi}O \ket{\psi}$, we deduce that $P_1$ ($P_0$ respectively) act as $q\times \Id$ ($(1-q)\times \Id$ respectively) on $\mathcal{H}$. As a result we have that, 
\begin{align}
    \Delta_0 Q^\dagger \Pi_1 Q \Delta_0 = (\Id \otimes \ket{0}) P_1 (\Id \otimes \bra{0}) = q\times \Delta_0 \label{eq:delta_action}
\end{align}
and similarly $\Delta_0 Q^\dagger \Pi_0 Q \Delta_0 = (1-q)\times \Delta_0$. Now let us iterate what will happen to the state throughout the procedure. After applying the unitary $Q$ on the state $\psi$ the state in hand would be the following, 
$$Q\ket{\psi}\ket{0} = \sqrt{q}\ket{1}\ket{\phi_1(\psi)}+ \sqrt{1-q}\ket{0}\ket{\phi_0(\psi)}$$

In case measuring $\Pi$ yields outcome $1$ we end up with the state $\ket{1}\ket{\phi_1(\psi)}$ which is exactly as desired. So let us assume the outcome is $0$. Now applying $Q^\dagger$, $2\Delta_0 - \Id$ and $Q$ consecutively we are left with the state 
\begin{align}
Q(2\Delta-1) Q^\dagger \ket{0}\ket{\phi_0(\psi)} &= \frac{1}{\sqrt{1-q}}Q(2\Delta_0 - 1) \Pi_0 Q\Delta_0 \ket{\psi}\ket{0}\label{eq:state_trans_mv1}\\
& = 2\sqrt{1-q} Q\ket{\psi}\ket{0} - \frac{1}{\sqrt{1-q}}\Pi_0 Q\ket{\psi}\ket{0} \label{eq:state_trans_mv2}\\ 
& = 2\sqrt{q(1-q)}\ket{1}\ket{\phi_1(\psi)} + (1-2q)\ket{1}\ket{\phi_0(\psi)}\label{eq:state_trans_mw}
\end{align}
Where the transition from \cref{eq:state_trans_mv1} to \cref{eq:state_trans_mv2} is due to \cref{eq:delta_action}. What matters, is that this vector is still in the two dimensional space spanned by $\ket{0}\ket{\phi_0(\psi)}$ and $\ket{1}\ket{\phi_1(\psi)}$ and measuring it with respect to $\Pi$ yields outcome $1$ and residual state $\ket{1}\ket{\phi_1(\psi)}$ with probability $4 q (1-q)$ and outcome $0$ and state $\ket{0}\ket{\phi_0(\psi)}$ with probability $(1-2q)^2$. Notice that if measuring $\Pi$ yields output $0$ again, the residual state would be $\ket{0}\ket{\phi_0(\psi)}$ and the state at the beginning of the next round would again be as described in \cref{eq:state_trans_mw}. Hence the probability of the procedure not outputting $1$ after $t+1$ repetitions is given by $(1-q)(1-2q)^{2t}$. Hence by setting $t = O(\log(1/\delta)\frac{1}{q(q-1)})$, this probability would be less than $\delta$. 

This allows us to conclude that with probability $1-\delta$, the adversary would have the state $\Pi_1 Q \ket{\psi}\ket{0}$ after running the procedure, which combined with \cref{eq:Q_V_distance}, shows that they have a state negligibly close to $\Pi_1 U \ket{\psi}\ket{0}$. \comm{KH}{write distance in terms of delta}
% This allows us to invoke \cref{lemma:output_state} which implies applying the unitary $U_{enc}^{\dagger}U_{dec}^{\dagger}U_{comp}^{\dagger}$ on the adversaries state, would leave the state at negligible distance from the state $\ket{\tilde{\psi}}$,
% \begin{align}
%     \ket{\tilde{\psi}} = \ket{pk}^{\otimes m}\sum_{b_1,\dots,b_m} \ket{b_1\dots b_m}_b\sum_{sk\in S_{1/\log(m)}}\ket{sk}_{sk}\ket{0}
% \end{align}
% where $S_{1/\log(m)}=\{sk| Pr_{b\sim U}[Dec(sk,Enc(pk,b)) = b]\geq 1-1/\log(m)\}$. All left to do for $\adv$ is to measure the $sk$ register to recover a secret key $sk^*$ on this state and on a challenge ciphertext ${ct}^*$, return $Dec(sk^*,{ct}^*)$. Due to the definition of $S_{\log(m)}$ the probability of $\adv$ decrypting $\hat{ct}$ correctly is $(1-\delta - \negl(\lambda))(1-\frac{1}{\log(m)})$. By setting $\delta \approx 1/2^{m}$, the probability of decrypting correctly would be significantly more than $1/2$. 

\noindent\textbf{Realizing unitary $V$}:\\
The only subtlety left is realizing the unitary $V$. We will explicitly use the fact that $\adv$ is computationally unbounded. Note that any unitary operator can be approximated to arbitrary accuracy with \textsf{CNOT}, Hadamard, phase and $\pi/8$ gates~\cite[Chapter 4.5]{DBLP:books/daglib/0046438}. Hence there exists a quantum circuit $C$, most likely inefficient, such that $C$ computes a unitary $\tilde{V}$ such that $|\tilde{V} - V| \leq O(2^{-2^{\lambda}})$, i.e. $\tilde{V}$ is doubly exponentially close to $V$. 

This would also imply that $\tilde{Q} = \tilde{V}U$ is $O(2^{-2^{\lambda}})$ close to $Q$ in operator distance. Hence, we can consider $\adv$ to be a non-uniform adversary who is given the description of the circuit $C$. So in reality $\adv$ will run the \textsf{get\_state} procedure with the unitary $\tilde{Q}$ instead of $Q$ and we prove that the output of the process is in fact negligibly close to $\Pi_1 Q\ket{\psi}\ket{0}$, hence negligibly close to the desired state $\Pi_1 U\ket{\psi}\ket{0}$. This is done similarly to the proof of the perturbed version of the quantum rewinding lemma from~\cite{DBLP:journals/siamcomp/Watrous09}. 

We bound the distance of the output of the procedure ran with $\tilde{Q}$ and $\Pi_1 Q\ket{\psi}\ket{0}$ using triangle inequality. At each iteration, the distance between the states, when running the algorithm with $\tilde{Q}$ or with $Q$ is bounded by $|\tilde{Q}-Q| = O(2^{-2^{\lambda}})$. To elaborate, let us call the states after the first iteration $\ket{\phi}$ and $\ket{\phi'}$. Now we have that $d(\ket{\phi} , \ket{\phi'})\leq O(2^{-2^{\lambda}})$, and we wish to bound the distance between $\tilde{Q}\ket{\phi}$ and $Q\ket{\phi'}$. This can be done as follows, 
\begin{align*}
    |Q\ket{\phi'} - \tilde{Q}\ket{\phi}| \leq |Q(\ket{\phi'}- \ket{\phi})|+ |(Q-\tilde{Q})\ket{\phi}|= O(2^{-2^{\lambda}})
\end{align*}
Where the first inequality follows from triangle inequality and the second from the distance bounds given in the previous paragraph. With the same argument, we can show that at each iteration the distance increases at most by $|Q-\tilde{Q}|$, hence by $O(2^{-2^{\lambda}})$. Hence after $t = O(\frac{1}{q(1-q)})$ iterations the distance would increase by $O(2^{\textsf{poly}(\lambda)})\times \theta(2^{-2^{\lambda}})$, as $\frac{1}{q(1-q)}= O(2^{\poly(\lambda)})$ which is still negligible in $\lambda$. This concludes the proof of \cref{lemma:generic_rewinding_lemma}.


\end{proof} 


==> proof_rewinding_redux.tex <==
% !TEX root = main.tex
\begin{proof}
We follow an approach similar to the proof of the quantum rewinding lemma from~\cite{DBLP:journals/siamcomp/Watrous09}.
We start by introducing some notation.
First, it is clear that by definition of~$p(\psi)$, for every state $\ket\psi \in \cH_\text{in}$, there are states~$\ket{\phi_b(\psi)} \in \cH_\text{in} \ot \cH_\text{work}$ for~$b\in\{0,1\}$ such that the following equation holds:
\begin{equation}\label{eq:U decomp}
  U \ket{\psi} \ket{0}^{\otimes\ell} \ket0
= \sqrt{1-p(\psi)} \ket{\phi_0(\psi)} \ket0 + \sqrt{p(\psi)} \ket{\phi_1(\psi)} \ket1
\end{equation}
Clearly, $\ket{\phi_0(\psi)}$ and~$\ket{\phi_1(\psi)}$ are uniquely defined if~$p(\psi)\neq1$ and~$p(\psi)\neq0$, respectively.
Next, we consider the POVM element corresponding to initializing work and output qubit in the~$\ket0$ state, applying the unitary, and then measuring the output qubit:
\begin{align}\label{eq:P}
    P :=
\parens*{ \Id \ot \bra0^{\ot\ell} \ot \bra0 } U^\dagger \parens*{ \Id \ot \Id \ot \proj1 } U \parens*{ \Id \ot \ket0^{\ot\ell} \ot \ket0 }
\end{align}
Fix an arbitrary eigenbasis~$\ket{\psi_k}$ of~$P$.
Then~$p_k := \angles{\psi_k | P | \psi_k} = p(\psi_k)$ is the corresponding eigenvalue.
We abbreviate $\ket{\phi_{b,k}} := \ket{\phi_b(\psi_k)}$ for $b\in\{0,1\}$.
Then,
\begin{align*}
  \braces[\big]{ \ket{\phi_{0,k}} \ket0 : p_k \neq 1 }
\cup \braces[\big]{ \ket{\phi_{1,k}} \ket1 : p_k \neq 0 }
\end{align*}
is an orthonormal basis of~$U \parens{ \cH_\text{in} \ot \ket{0}^{\otimes\ell} \ot \ket0 }$,
as follows from \cref{eq:U decomp} and the unitarity of~$U$.
% Since $\dim\cH_\text{in} \leq \dim (\cH_\text{in} \ot \cH_\text{work})$,
Furthermore, we can choose~$\ket{\phi_{0,k}} \in \cH_\text{in} \ot \cH_\text{work}$ for~$p_k=1$ and~$\ket{\phi_{1,k}} \in \cH_\text{in} \ot \cH_\text{work}$ for~$p_k=0$ arbitrarily, and in particular such that
\begin{align*}
  \mathcal B := \braces[\big]{ \ket{\phi_{0,k}} \ket0 }
\cup \braces[\big]{ \ket{\phi_{1,k}} \ket1 }
\end{align*}
is orthonormal.
Thus we may define a unitary~$V$ on~$\cH$ that acts as
\begin{align}\label{eq:V}
  &V \parens{ \sqrt{1-p_k} \ket{\phi_{0,k}} \ket0 + \sqrt{p_k} \ket{\phi_{1,k}} \ket1 }
= \sqrt{1-q} \ket{\phi_{0,k}} \ket0 + \sqrt{q} \ket{\phi_{1,k}} \ket1, \\
\nonumber
  &V \parens{ -\sqrt{p_k} \ket{\phi_{0,k}} \ket0 + \sqrt{1-p_k} \ket{\phi_{1,k}} \ket1 }
= -\sqrt{q} \ket{\phi_{0,k}} \ket0 + \sqrt{1-q} \ket{\phi_{1,k}} \ket1,
\end{align}
on the span of~$\mathcal B$, and by the identity on the orthogonal complement.
We may think of~$V$ as a ``correction'' unitary, in the sense that while each~$\ket{\psi_k}$ is an eigenvector of~$P$ with eigenvalue~$p_k$, they are all eigenvectors with eigenvalue~$q$ of the operator
\begin{align*}
    Q := \parens*{ \Id \ot \bra0^{\ot\ell} \ot \bra0 }
    W^\dagger \parens*{ \Id \ot \Id \ot \proj1 } W
    \parens*{ \Id \ot \ket0^{\ot\ell} \ot \ket0 },
\end{align*}
which is defined as in \cref{eq:P} but with $W := VU$ in place of~$U$.
Indeed, it follows from \cref{eq:U decomp,eq:V} that
$\angles{\psi_k | Q | \psi_l}
% = \bra{\psi_k} \bra0^{\ot\ell} \bra0 U^\dagger V^\dagger \parens*{ \Id \ot \Id \ot \proj1 } V U \ket{\psi_l} \ket0^{\ot\ell} \ket0
% = \parens*{ \sqrt{1-q} \bra{\phi_{0,k}} \bra0 + \sqrt{q} \bra{\phi_1(\psi_k)} \bra1 } \parens*{ \Id \ot \Id \ot \proj1 } \parens*{ \sqrt{1-q} \ket{\phi_0(\psi_l)} \ket0 + \sqrt{q} \ket{\phi_1(\psi_l)} \ket1 } \\
= q \, \angles{\phi_{1,k} | \phi_{1,l}}
= q \delta_{k,l}$,
since the $\ket{\phi_{1,k}}$ are orthonormal, and hence~$Q = q \Id_\text{in}$.

Next, we prove that~$V$ is close to the identity and hence~$W=VU$ is close to~$U$.
Indeed, $V$ only acts nontrivially on the span of~$\mathcal B$, where it is block-diagonal with respect to the two-dimensional subspaces spanned by~$\ket{\phi_{0,k}} \ot \ket0, \ket{\phi_{1,k}} \ot \ket1$, each on which by \cref{eq:V} it acts
\begin{align*}
  % \begin{pmatrix}\sqrt{1-q} & -\sqrt{q} \\ \sqrt{q} & \sqrt{1-q} \end{pmatrix}
  % \begin{pmatrix} \sqrt{1-p_k} & -\sqrt{p_k} \\ \sqrt{p_k} & \sqrt{1-p_k} \end{pmatrix}^T
% = \begin{pmatrix} \sqrt{1-q} & -\sqrt{q} \\ \sqrt{q} & \sqrt{1-q} \end{pmatrix}
%   \begin{pmatrix} \sqrt{1-p_k} & \sqrt{p_k} \\ -\sqrt{p_k} & \sqrt{1-p_k} \end{pmatrix}
% = \begin{bmatrix} \sqrt{(1-q)(1-p_k)} + \sqrt{qp_k} & \quad \sqrt{(1-q)p_k} - \sqrt{q(1-p_k)} \\
%   \sqrt{q(1-p_k)} - \sqrt{(1-q)p_k} & \quad \sqrt{(1-q)(1-p_k)} + \sqrt{qp_k} \end{bmatrix} =
\begin{bmatrix} \sqrt{1-\eps_k^2} & \eps_k \\
  -\eps_k & \sqrt{1-\eps_k^2} \end{bmatrix},
\end{align*}
with $\eps_k = \sqrt{(1-q)p_k} - \sqrt{(1-p_k)q}$.
Since $\abs{\eps_k} \leq \negl(\lambda)$ by assumption, we have
\begin{align}\label{eq:W_U_distance}
  \norm{W - U}
\leq \norm{V - I}
= \max_k \norm*{
  \begin{bmatrix} \sqrt{1-\eps_k^2} - 1 & \eps_k \\
  -\eps_k & \sqrt{1-\eps_k^2} - 1 \end{bmatrix}}
\leq \negl(\lambda)
\end{align}
The original rewinding lemma uses the bound in \cref{eq:W_U_distance} to bound the distance of the output state from the desired state.
However, in our case the process may need to be rewound exponentially many times, in which case this additive error might end up being non-negligible.
The way by which we circumvent this is by replacing~$U$ with~$W=VU$ \emph{in the rewinding procedure}.
To this end we need to implement the unitary~$V$.
While this procedure may in general not be efficient, we do not care about efficiency for the purposes of the lemma.
We will discuss how~$V$ (and $V^\dagger$) can be implemented in detail towards the end of the proof, but for now we assume we  are given implementations of the unitaries~$V$ and~$V^\dagger$ and describe the procedure that achieves the desired behavior.
Given an arbitrary state of the form~$\ket\psi\ket0^{\ot\ell}\ket0$ and a parameter~$\delta>0$ to be chosen later\MW{It is not currently chosen.}, it proceeds as follows:
\begin{enumerate}
  \item Set $t=0$.
  \item Apply $W=VU$.
  \item While $t \leq O(\frac{\log(1/\delta)}{q(1-q)})$:
  \begin{enumerate}
    \item Measure the output qubit in the computational basis.
    \item If the outcome is~$1$, return. Otherwise continue.
    \item Apply $W^\dagger = U^\dagger V^\dagger$.
    \item Apply the unitary $2 \Delta - \Id$, where $\Delta := \Id \ot \proj0^{\ot\ell} \ot \proj0$.
    \item Apply $W = V U$.
    \item Set $t = t+1$.
  \end{enumerate}
\end{enumerate}
It is clear that the above can be implemented by a quantum circuit.
We claim that with probability at least~$\geq 1-\delta$, it returns the state
\begin{align*}
  \frac1{\sqrt q} \parens{ \Id \ot \Id \ot \proj1 } W \ket\psi\ket0^{\ot\ell}\ket0.
\end{align*}
To see this, we analyze what happens to the state throughout the procedure.
After applying the unitary~$W$ on the initial state, we obtain a state of the form
\begin{align}\label{eq:W action}
  W \ket\psi\ket0^{\ot\ell}\ket0
= \sqrt{1-q}\kett{\tilde\phi_0(\psi)}\ket{0} + \sqrt{q}\kett{\tilde\phi_1(\psi)}\ket{1},
\end{align}
where the amplitudes follow from~$Q = q \Id_\text{in}$, which we established above.
We now enter the loop body and measure the last qubit.
If the outcome is~1, we end up with the desired state $\kett{\tilde\phi_1(\psi)}\ket{1}$ and this happens with probability~$q$.
Let us assume that the outcome is~0, which happens with probability~$1-q$.
Then the state at the end of the loop body is given by
\begin{align*}
&\quad W(2\Delta - \Id)W^\dagger \kett{\tilde\phi_0(\psi)}\ket{0}
= 2 W \Delta W^\dagger \kett{\tilde\phi_0(\psi)}\ket{0} - \kett{\tilde\phi_0(\psi)}\ket{0} \\
&= \frac2{\sqrt{1-q}} W \Delta W^\dagger \parens{ \Id \ot \Id \ot \proj0 } W \Delta \ket\psi\ket0^{\ot\ell}\ket0 - \kett{\tilde\phi_0(\psi)}\ket{0} \\
&= 2 \sqrt{1-q} \, W \ket\psi\ket0^{\ot\ell}\ket0 - \kett{\tilde\phi_0(\psi)}\ket{0} \\
% &= 2 \sqrt{1-q} \parens*{ \sqrt{1-q}\kett{\tilde\phi_0(\psi)}\ket{0} + \sqrt{q}\kett{\tilde\phi_1(\psi)}\ket{1} } - \kett{\tilde\phi_0(\psi)}\ket{0} \\
&= (1 - 2q) \kett{\tilde\phi_0(\psi)}\ket{0} + 2 \sqrt{q(1-q)} \kett{\tilde\phi_1(\psi)}\ket{1},
\end{align*}
where the third line holds since we have $Q = q \Id_\text{in}$ and hence %$\Delta W^\dagger \parens{ \Id \ot \Id \ot \proj1 } W \Delta = q \Id_\text{in} \ot \proj0^{\ot\ell} \ot \proj0$ and
$\Delta W^\dagger \parens{ \Id \ot \Id \ot \proj0 } W \Delta = (1-q) \Id_\text{in} \ot \proj0^{\ot\ell} \ot \proj0$, and the last step uses \cref{eq:W action}.
Importantly, just like \cref{eq:W action} this vector is still in the two-dimensional subspace spanned by $\kett{\tilde\phi_0(\psi)}\ket{0}$ and $\kett{\tilde\phi_1(\psi)}\ket{1}$.
Thus the same analysis as above applies to the next iteration, except that now the probability of outcome~0 is $(1-2q)^2$, and this continues to be so for all further iterations.
It follows that the failure probability of not returning (with the desired state) within~$T$ iterations is given by $(1-q)(1-2q)^{2T}$.
By choosing $T = O(\frac{\log(1/\delta)}{q(1-q)})$ as above, this probability can be made less than~$\delta$.
\MW{Should assume $q\neq1$.}
Thus we have established the claim that with probability at least~$1-\delta$, the above procedure returns the desired state~$\kett{\tilde\phi_1(\psi)} \ket 1 = \frac1{\sqrt q} \parens{ \Id \ot \Id \ot \proj1 } W \ket\psi\ket0^{\ot\ell}\ket0$.
\MW{$W$ is negligibly close to~$U$, but we need to divide by $\sqrt{q}$?!}
\MW{Translate into a fidelity/trace distance statement.}

\MW{Still need to read the following.}
\noindent\textbf{Realizing unitary $V$}:\\
The only subtlety left is realizing the unitary $V$. We will explicitly use the fact that $\adv$ is computationally unbounded. Note that any unitary operator can be approximated to arbitrary accuracy with \textsf{CNOT}, Hadamard, phase and $\pi/8$ gates~\cite[Chapter 4.5]{DBLP:books/daglib/0046438}. Hence there exists a quantum circuit $C$, most likely inefficient, such that $C$ computes a unitary $\tilde{V}$ such that $|\tilde{V} - V| \leq O(2^{-2^{\lambda}})$, i.e. $\tilde{V}$ is doubly exponentially close to $V$.

This would also imply that $\tilde{W} = \tilde{V}U$ is $O(2^{-2^{\lambda}})$ close to $W$ in operator distance. Hence, we can consider $\adv$ to be a non-uniform adversary who is given the description of the circuit $C$. So in reality $\adv$ will run the \textsf{get\_state} procedure with the unitary $\tilde{W}$ instead of $W$ and we prove that the output of the process is in fact negligibly close to $\Pi_1 W\ket{\psi}\ket{0}$, hence negligibly close to the desired state $\Pi_1 U\ket{\psi}\ket{0}$. This is done similarly to the proof of the perturbed version of the quantum rewinding lemma from~\cite{DBLP:journals/siamcomp/Watrous09}.

We bound the distance of the output of the procedure ran with $\tilde{W}$ and $\Pi_1 W\ket{\psi}\ket{0}$ using triangle inequality. At each iteration, the distance between the states, when running the algorithm with $\tilde{W}$ or with $W$ is bounded by $|\tilde{W}-W| = O(2^{-2^{\lambda}})$. To elaborate, let us call the states after the first iteration $\ket{\phi}$ and $\ket{\phi'}$. Now we have that $d(\ket{\phi} , \ket{\phi'})\leq O(2^{-2^{\lambda}})$, and we wish to bound the distance between $\tilde{W}\ket{\phi}$ and $W\ket{\phi'}$. This can be done as follows,
\begin{align*}
    |W\ket{\phi'} - \tilde{W}\ket{\phi}| \leq |W(\ket{\phi'}- \ket{\phi})|+ |(W-\tilde{W})\ket{\phi}|= O(2^{-2^{\lambda}})
\end{align*}
Where the first inequality follows from triangle inequality and the second from the distance bounds given in the previous paragraph. With the same argument, we can show that at each iteration the distance increases at most by $|W-\tilde{W}|$, hence by $O(2^{-2^{\lambda}})$. Hence after $t = O(\frac{1}{q(1-q)})$ iterations the distance would increase by $O(2^{\textsf{poly}(\lambda)})\times \theta(2^{-2^{\lambda}})$, as $\frac{1}{q(1-q)}= O(2^{\poly(\lambda)})$ which is still negligible in $\lambda$. This concludes the proof of \cref{lemma:generic_rewinding_lemma}.

\end{proof}


==> sec_generic_lemma.tex <==
% !TEX root = main.tex
The last component of the proof of \cref{thm:impossibility} is to show that there exists a process which given $U$ and $\ket{\pk}^{\otimes m}$ terminates with a residual state in negligible distance from $\Pi_1 U\ket{\pk}^{\otimes m}\ket{0}$ with a high probability.

We start by stating a generalized version of the quantum rewinding lemma from \cite{DBLP:journals/siamcomp/Watrous09}. The main addition to the standard lemma is that our lemma allows an unbounded number of rewinds without increasing the distance of the residual state from the desired state. We note that this lemma might be of interest on its own as it provides a generic framework for proving lower bounds of the same flavor.

\begin{lemma}[Unbounded Quantum Rewinding, restated \cref{lem:unbounded watrous intro}]\label{lemma:generic_rewinding_lemma}%
\unboundedWatrous
\end{lemma}

\MW{I'm working on a re-rendering of the proof (commented out until complete).}
% \input{proof_rewinding_redux}
\MW{Original proof from here on.}

Before proving the result we start with a simple lemma that mainly serves to introduce some notation.

\begin{lemma}\label{lemma:orthonormal_basis}
Let $\mathcal{H}$ be a Hilbert space, $U$ a unitary acting on $\mathcal{H}\otimes (\mathbb{C}^{2})^{\otimes l}$ and $\Pi$ a rank one projective measurement on the same space. Let $\{\psi_i\}_{i \in [1,\dots,k]}$ be an orthonormal basis of $\mathcal{H}$ consisting of eigenvectors of the operator $P$,
\begin{align*}
    P =  (\Id \otimes \bra{0})^{\dagger} U^{\dagger} \Pi_1 U (\Id \otimes \ket{0})
\end{align*}
And for all $i$, define $ p(\psi_i) = \bra{\psi_i} P \ket{\psi_i}$. define $\phi_b(\psi_i)$ such that
$$U (\Id\otimes \ket{0})\ket{\psi_i} = \sqrt{p(\psi_i)} \ket{1}\ket{\phi_1(\psi_i)} + \sqrt{1-p(\psi_i)}\ket{0}\ket{\phi_0(\psi_i)}$$

$\{\ket{0}\ket{\phi_0(\psi_i)}\}\cup \{\ket{1}\ket{\phi_1 (\psi_i)}\}$ induces an orthonormal basis for  $\textsf{Sup} [U(\Id \otimes \ket{0})]\subseteq\mathcal{H}\otimes (\mathbb{C}^{2})^{\otimes l}$.
\end{lemma}
\begin{proof}
The proof of this lemma is quite simple. We first prove that for $i\neq j$, $\langle \phi_0(\psi_i)| \phi_0(\psi_j) \rangle= 0$. This follows from the following transition,
\begin{align*}
    0 = \bra{\psi_i} (\Id \otimes \bra{0}) U^\dagger \Pi_0 U(\Id\otimes \ket{0}) \ket{\psi_k} = \sqrt{p(\psi_i)p(\psi_j)} \langle{\phi_0(\psi_i)} | {\phi_0(\psi_j)}\rangle
\end{align*}
Same holds for $\langle{\phi_1(\psi_i)}|{\phi_1(\psi_j)}\rangle$ for $i\neq j$. Moreover for all
$i,j$ $$\bra{\phi_0(\psi_i)}\bra{0} \ket{1}\ket{\phi_1(\psi_j)} = 0$$ This concludes that the elements of the basis are orthonormal (the vectors are by definition units).

\qed
\end{proof}

Provided the notation from this lemma we proceed to prove \cref{lemma:generic_rewinding_lemma}.
\input{proof_rewinding_lemma}
\subsection{Proving \cref{thm:impossibility}}
Given \cref{lemma:generic_rewinding_lemma} we are provided with all the tools required to prove \cref{thm:impossibility}. This boils down to putting lemmas proven in \cref{sec:impossibility} and the unbounded rewinding lemma together. Let us proceed with the proof.
\begin{proof}[\cref{thm:impossibility}]
    Given any QPKE $\Pi$, we describe an unbounded, non-uniform adversary which breaks the IND-CPA security. The adversary works as follows. Starting from the state $\ket{\psi}=\ket{pk}^{\otimes m}$, they implement the unitary $U$ from \cref{def:unitary_PKE}. The goal is to apply \cref{lemma:generic_rewinding_lemma} to $U$ and $\ket{\psi}$.

    To do so we require to prove the two requirements of the lemma. Let $\mathcal{H}$ be the Hilbert space spanned by $\ket{pk}^{\otimes m}$ for all honestly generated public-keys $\ket{pk}^{\otimes m}$. Setting $q = \frac{1}{2^m}$, \cref{lemma:success_prob} shows that for all $\ket{\psi} \in \mathcal{H}$, $|p_1(\psi)-q| = \neg(\lambda)$. Moreover $\frac{1}{q(1-q)}$ is $O(2^{\poly(\lambda)})$. Invoking \cref{lemma:generic_rewinding_lemma}, we have that there exists a procedure that halts, and the output state of the procedure is in negligible distance from $(\Pi_1\otimes \id )U\ket{\psi}\ket{0}$.

    After running the procedure described in \cref{lemma:generic_rewinding_lemma}, the adversary inverts $U_{comp}$, $U_{dec}$ and $U_{enc}$ and measures the secret-key register. Now according to \cref{lemma:output_state} the obtain secret-key will be in set $S_{\frac{1}{\log(m)}}$ with probability $1-\neg(\lambda)$. Hence,
    \begin{equation}
        Pr_{b\sim U}[Dec(Enc(b,pk),sk) = b] \geq 1-\frac{1}{\log(m)}
    \end{equation}
    This concludes the proof, as the challenge plaintext is also picked uniformly at random, hence the advantage of this adversary is significantly more than $1/2$.


\end{proof}


==> sec_impossiblity_prs.tex <==
% !TEX root = main.tex
The last contribution of this work is showing how our framework using the unbounded rewinding lemma can be used to provide a novel proof for an already known result, i.e. impossibility of information theoretically secure pseudo-random state constructions. 

We start by briefly defining what a pseudo-random state family is. Later we define the unitary $U_{PRS}$ which \cref{lemma:generic_rewinding_lemma} will be applied to and prove the analogous lemmas to \cref{lemma:output_state,lemma:success_prob} for $U_{PRS}$.

\begin{definition}[Pseudo-random state family]
A pseudo-random state family (PRS) is ..  
\end{definition}

The main theorem of this section is as follows. 
\begin{theorem}\label{thm:prs_impossibility}
    There does not exist any pseudo-random state family which is information-theoretically indistinguishable from Haar random.
\end{theorem}

Let us start by giving a high-level intuition of the attack, followed by the description of the unitary $U_{PRS}$. Given $2m$ copies of a pseudo-random state $\ket{\psi_{sk^*}}$ or $m$ copies of a random Haar state, the goal is to apply a generic key guessing attack. What we mean by this is following the upcoming approach:\\

\noindent\underline{\textsf{get\_sk}}

\begin{enumerate}
    \item Start with the state $\ket{\psi}^{\otimes m}$. Let us call it the PRS register
    \item Attach a uniform superposition of secret keys guess $\sum_{sk}\ket{sk}_{sk}$\label{alg:prs_init}
    \item Controlled on the $sk$ register apply $(U_{sk}^{\otimes m})^{\dagger}$ on the PRS register. \label{alg:prs_controlled}
    \item Add an ancilla qubit and apply a unitary which sets it to one if all the PRS register is $0$ \label{alg:prs_check}
    \item Measure the ancilla register and if the outcome is $1$ revert step~\ref{alg:prs_controlled} and measure the $sk$ register to get a secret key $\Tilde{sk}$
    \item If the outcome is $0$ rewind 
\end{enumerate}
Now given a decent secret key candidate $\Tilde{sk}$ the adversary proceeds as follows:\\


\noindent\underline{\textsf{distinguish}}
\begin{enumerate}
    \item Compute $m$ copies of $\ket{\psi_{\Tilde{sk}}}$, i.e. a pseudo-random state generated with key $\Tilde{sk}$
    \item Perform $m$ swap-test between $\ket{\psi}$ and $\ket{\psi_{\tilde{sk}}}$
\end{enumerate}

Unitary $U_{PRS}$ will be handling steps~\ref{alg:prs_init},~\ref{alg:prs_controlled} and~\ref{alg:prs_check}. So we define three unitaries $U_{init}$, $U_{invert}$ and $U_{check}$ which act as follows, 
\begin{align}
    U_{init}\ket{\psi}_{PRS}\ket{0}_{sk}\ket{0}_{out} = \sum_{sk}\ket{\psi}_{PRS}\ket{sk}_{sk}\ket{0}_{out}\\
    U_{invert} \ket{\psi}\ket{sk}\ket{0} = (U_{sk}^{\dagger}\otimes \id \otimes \id)\ket{\psi}\ket{sk}\ket{0} \\ 
    \forall \text{ states }\mathcal{E}, U_{check} \ket{0}\ket{\mathcal{E}}\ket{0} = \ket{0}\ket{\mathcal{E}}\ket{1}\\ 
    \forall \text{ states }\mathcal{E}, \text{ basis vector } x\neq 0, U_{check} \ket{x}\ket{\mathcal{E}}\ket{0} = \ket{0}\ket{\mathcal{E}}\ket{0}
\end{align}

$U$ is defined to be $U_{check}\circ U_{invert}\circ U_{init}$. Let $\Pi_1 = \id\otimes \id \otimes \ket{0}\bra{0}_{out}$ and $\Pi_0 = \id - \Pi_1$, the goal is to find a state close to $\Pi_1 U \ket{\psi}^{\otimes m} \ket{0}\ket{0}$ for the challenge state $\ket{\psi}$. To do so, we continue by proving conditions required by \cref{lemma:generic_rewinding_lemma}.

\begin{lemma}\label{lemma:prs_success_prob}
Let $\Gamma$ be a PRS family and define $\mathcal{H} \subseteq \mathbb{C}^{\otimes nm}$ to be the space spanned by all $\{\ket{\psi_{sk}}^{\otimes m}\}_{sk\gets \Gamma.\textsf{key\_gen}(1^{\lambda})}$. Let $U$ be as defined above. For all $\ket{\psi}\in \mathcal{H}$ define $p(\psi)$ and $\phi_b(\psi)$ as follows, 
\begin{align*}
    U\ket{\psi}\ket{0}\ket{0} = \sqrt{1-p(\psi)}\ket{\phi_0(\psi)} + \sqrt{p(\psi)}\ket{\phi_1(\psi)}
\end{align*}
For all $\ket{\psi} \in \mathcal{H}$ we have that,
\begin{equation}
    |p(\psi) - \frac{1}{2^{2mn}}| = \negl(\lambda)
\end{equation}
\end{lemma}
\begin{proof}
For the sake of simplicity, we assume $m =1$. Whenever there are $m$ copies of the state the probability $p(\psi)$ is powered by $m$ as the states are in tensor. As before we only prove this for the basis vectors, i.e. $\ket{\psi} = \ket{\psi_{sk^*}}$. Now note that $p(\psi) = \trace[(\id \otimes \id \otimes \ket{1}\bra{1}_{out}) U\ket{\psi}\ket{0}\ket{0}]$. Looking at what $out$ contains this is equal to probability of measuring $0$, when measuring the $U_{sk}^{\dagger}\ket{\psi}$ in computational basis for a uniformly picked $sk$, i.e. $E_{sk}[\bra{\psi}U_{sk} \ket{0}\bra{0}U_{sk}^{\dagger}\ket{\psi}]$

One can notice that as $\ket{\psi}$ is a PRS, on average over $sk$ we have:
\begin{align}
   \bra{0}U_{sk}^{\dagger}\ket{\psi} \approx_{\negl} \bra{0}U_{sk}^{\dagger}\ket{\psi_R}
\end{align}
Notice that $U_{sk}\ket{0}$ is also a pseudo-random state hence we deduce
\begin{align}
    E_{sk}[\bra{0}U_{sk}^{\dagger}\ket{\psi_R}] &\approx_{\negl} E_{\ket{\psi_{R'}}\gets \mu}[\langle{\psi_{R'}}| \psi_R\rangle]\\
   & = E_{Q' \gets \mu}[\bra{\psi_0}Q'^{\dagger} Q\ket{\psi_0}]
\end{align}
where $\ket{\psi} = Q\ket{\psi_0}$ for a fiducial state $\ket{\psi_0}$. As $Q'$ is Haar random, so is $Q'^\dagger Q$ hence we can rewrite the equation as follows.
\begin{align}
    E_{sk}[\bra{0}U_{sk}^{\dagger}\ket{\psi_R}] &\approx_{\negl}  E_{Q'' \gets \mu}[\bra{\psi_0}Q''\ket{\psi_0}]\\
    &= \int dQ'' \bra{\psi_0} Q'' \ket{\psi_0} = \bra{\psi_0} \int dQ'' Q'' \ket{\psi_0} \\
    &= \bra{\psi_0} 1/2^n\id \ket{\psi_0}  = 1/{2^n}
\end{align}
\todo[inline]{I think $2^{-2n}$ is actually correct. somehow this is the same as having two unitaries that act the same and the dimension of the unitaries is $2^{2n}$}
This concludes that the probability of measuring $0$ after applying $U_{sk}$ on $\ket{\psi}$ is in negligible distance from $2^{-2n}$ on average over $sk$. 

\end{proof}

\begin{lemma}\label{lemma:prs_final_state}
Let $\Pi$, $\mathcal{H}$ be as defined in \cref{lemma:prs_success_prob}. Moreover, let $\Pi_1 = \ket{1}\bra{1}_{out}\otimes \id$ and $U_{PRS}$ as defined before. Let $\ket{\psi_{fin}} =   \Pi_1 U_{PRS}\ket{\psi_{sk^*}}^{\otimes m} \ket{0}$, where $\ket{\psi_{sk^*}}$ is the pseudo-random state generated with key $sk^*$. We have that $\ket{\psi_{fin}}$ is in negligible distance from $\ket{\tilde{\psi}}$, 
\begin{align}
    \ket{\tilde{\psi}} = \ket{sk^*}\ket{0}^{\otimes m}\ket{1}
\end{align}
\end{lemma}
\todo[inline]{I'm not sure the proof for the lemma works as it is stated}
\begin{proof}
We take a similar approach to the proof of \cref{lemma:output_state}. We can write $U_{init}\ket{\psi}_{PRS}\ket{0}$ as, 
\begin{align}
    \sum_{sk\neq sk^*} \ket{sk}\ket{\psi_{sk}}^{\otimes m}\ket{0} + \ket{sk^*}\ket{\psi_{sk^*}}^{\otimes m}\ket{0}
\end{align}
Applying the unitaries $U_{invert}$ we get to the state,
\begin{align}
    \sum_{sk\neq sk^*} \ket{sk}U_{sk}^{\dagger,\otimes m}\ket{\psi_{sk^*}}^{\otimes m}\ket{0} + \ket{sk^*}U_{sk^*}^{\dagger,\otimes m}\ket{\psi_{sk^*}}^{\otimes m}\ket{0}\\ 
    =_{\negl} \sum_{sk\neq sk^*} \ket{sk}U_{sk}^{\dagger,\otimes m}\ket{\psi_R}^{\otimes m}\ket{0} + \ket{sk^*}\ket{0}\ket{0}\\
    =\underbrace{ \sum_{sk\neq sk^*} \ket{sk}U_{sk}^{\dagger,\otimes m}U_R^{\otimes m}\ket{0}\ket{0}_{out}}_{\ket{\psi_1}\ket{0}_{out}} + \underbrace{\ket{sk^*}\ket{0}\ket{0}_{out}}_{\ket{\psi_0}\ket{0}_{out}}
\end{align}
Where $\ket{\psi_R}$ and $U_R$ are Haar random states and unitaries respectively. Let us now consider the projection $M_0 = \ket{0}\bra{0}^{\otimes m}_{PRS} \otimes \id$. With respect to this projection, the state $\ket{\psi_1}\ket{0}+\ket{\psi_0}\ket{0}$ can be rewritten as, 
\begin{align}
    \ket{\psi_1}\ket{0}+\ket{\psi_0}\ket{0} = M_0 \ket{\psi_1}\ket{0} + (\id - M_0)\ket{\psi_1}\ket{0} + M_0\ket{\psi_0} \ket{0}
\end{align}
Now applying $U_{check}$ on this state and applying the projector $\Pi_1$ we are left with, 
\begin{align}
   \Pi_1(M_0 \ket{\psi_1}\ket{1} + (\id - M_0)\ket{\psi_1}\ket{0} + M_0\ket{\psi_0} \ket{1})\\ 
   = (M_0 \ket{\psi_1} + \ket{\psi_0})\ket{1}
\end{align}
The goal now would be to show that $M_0\ket{\psi_1}$ has a negligible norm, i.e. that $\bra{0}\bra{\psi_1} M_0\ket{\psi_1}\ket{0}$ is negligible. This is done as follows: 
\begin{align}
    \bra{0}\bra{\psi_1} M_0\ket{\psi_1}\ket{0} = \\\sum_{sk\neq sk^*}\bra{0} \bra{0} U_{sk}^{\otimes m}{U_R^\dagger}^{\otimes m}\bra{sk} M_0 \ket{sk}{U_{sk}^{\dagger}}^{\otimes m}U_R^{\otimes m}\ket{0}\ket{0}\\ 
    = \sum_{sk \neq sk^*} (\bra{0}_{PRS} {U_{sk}^{\dagger}}^{\otimes m}U_R^{\otimes m}\ket{0})
\end{align}
In the proof of \cref{lemma:prs_success_prob} we have already established that $(\bra{0}_{PRS} {U_{sk}^{\dagger}}^{\otimes m}U_R^{\otimes m}\ket{0})$ is $O(2^{-mn})$ on average over $sk$, hence, summing over $2^n$ values of $sk$ we have that $\bra{0}\bra{\psi_1} M_0\ket{\psi_1}\ket{0} = O(2^{n}\times 2^{-mn})$ which is negligible considering $m$ is considered to be $\poly(n)$. This concludes the proof. 
\end{proof}

Given \cref{lemma:prs_final_state,lemma:prs_success_prob} we can prove \cref{thm:prs_impossibility}.

